Explainable Black-Box Attacks Against Model-based Authentication

Establishing unique identities for both humans and end systems has been an active research problem in the security community, giving rise to innovative machine learning-based authentication techniques. Although such techniques offer an automated method to establish identity, they have not been vetted against sophisticated attacks that target their core machine learning technique. This paper demonstrates that mimicking the unique signatures generated by host fingerprinting and biometric authentication systems is possible. We expose the ineffectiveness of underlying machine learning classification models by constructing a blind attack based around the query synthesis framework and utilizing Explainable-AI (XAI) techniques. We launch an attack in under 130 queries on a state-of-the-art face authentication system, and under 100 queries on a host authentication system. We examine how these attacks can be defended against and explore their limitations. XAI provides an effective means for adversaries to infer decision boundaries and provides a new way forward in constructing attacks against systems using machine learning models for authentication.

==> images/facepp_mat.tex <==
% !TEX root = ../ms.tex
\begin{figure} 
	\centering

	\textsc{Face++ API}\par\medskip
  	\text{VAE Latent Space Perturb. Attack Coverage}\par\medskip
	\includegraphics[width=0.47\textwidth]{images/vae_tabular_mat_facepp.pdf}

	\caption{Coverage heatmaps for the Face++ Black-box experiment. Cells denote authentication success for each adversary--victim pair.}
	\label{fig:facepp_mat}
	% Without LIME, the VAE appraoch is more successful than random perturbations. In both cases, the LIME-assisted attack yields higher attack coverage. 

\end{figure}


==> images/forest_mattbl.tex <==
% !TEX root = ../ms.tex
\begin{figure}[t]
%\begin{minipage}[\textheight]{\linewidth}
%\parbox[t]{0.48\textwidth}{
%\begin{figure}[t]
%\begin{figure}[t] 
	\centering

\textsc{Random Forest}

\subfloat[][Random Pixel Image Perturb. Attack Coverage]{\includegraphics[width=0.978\columnwidth]{images/rand_image_mats_forest.pdf}}

\subfloat[][VAE Latent Space Perturb. Attack Coverage]{\includegraphics[width=0.978\columnwidth]{images/vae_tabular_mats_forest.pdf}}

    % \begin{subfigure}[t]{0.42\textwidth}
    %     \centering
    %     \text{Random Pixel Image Perturb.}
    %     \text{Attack Coverage}\par\medskip
    %     \includegraphics[width=\textwidth]{images/rand_image_mats_forest.eps}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.42\textwidth}
    %     \centering
    %     \text{VAE Latent Space Perturb.}
    %     \text{Attack Coverage}\par\medskip
    %     \includegraphics[width=\textwidth]{images/vae_tabular_mats_forest.eps}
    % \end{subfigure}

	% \textbf{(b)}\par\medskip
%    \captionsetup{width=\textwidth}
	\captionof{figure}{Coverage maps for the Facenet-RF classifier. Cells denote authentication success for each adversary--victim pair. Lighter cells denote unsuccessful queries shaded by the model's confidence, when available. }
	\label{fig:forest_mats}
	% Without LIME, the VAE appraoch is more successful than random perturbations. In both cases, the LIME-assisted attack yields higher attack coverage. 
%\end{figure}
\par\medskip
\hfill

%\begin{table}[b]
% \setlength\tabcolsep{3pt}
%\footnotesize
\centering
%\begin{subtable}{0.5\textwidth}
%\centering

\begin{footnotesize}
\begin{tabular}{|c||c|c|c|}
%\begin{tabular}{|c||cc|cc|cc|}
%\hline
% & \multicolumn{3}{c|}{Defenses} \\\hline
\multicolumn{4}{c}{Random Pixel Image Perturb. Attack} \\\hline
          & No Defenses                 & Random Defense              & All Defense\\\hline\hline
%          & Defense & Defense & Defenses \\\hline\hline
 Random   &  94 $\pm$ 64.82      &  ---                         &  ---  \\
  & $P(M)=73$\% & & \\\hline
 Ablation &  152.47 $\pm$ 84.10 &  162.33 $\pm$ 67.12  &  107.5 $\pm$ 18.27   \\
 & $P(M)=100$\% & $P(M)=100$\% & $P(M)=93$\% \\\hline
 LIME     &  120.67 $\pm$ 80.49 &  118.53 $\pm$ 26.26  &  123.71 $\pm$ 24.58   \\
 & $P(M)=100$\% & $P(M)=100$\% & $P(M)=93$\% \\\hline
\multicolumn{4}{c}{} \\
\multicolumn{4}{c}{VAE Latent Space Perturb. Attack} \\\hline
          & No Defense                 & Random Defense      & All Defense\\\hline\hline
%          & Defense & Defense & Defenses \\\hline\hline
 Random   &  84.11 $\pm$ 66.32  &  ---                         &  ---    \\
 & $P(M)=60$\% & & \\\hline
 Ablation &  125.23 $\pm$ 38.94 &  112.58 $\pm$ 50.37   &  102.43 $\pm$ 23.63   \\
 & $P(M)=87$\% & $P(M)=80$\% & $P(M)=93$\% \\\hline
 LIME     &  132.43 $\pm$ 35.04 &  99 $\pm$ 21.51       &  112.29 $\pm$ 39.27   \\
 & $P(M)=93$\% & $P(M)=80$\% & $P(M)=93$\% \\\hline

\end{tabular}
\end{footnotesize}
\par\medskip

\captionof{table}{The average number of adversarial queries before success in each of three experiments,
against the Facenet-RF classifier and with varying level of defenses at 30\% knowledge.
Dashes indicate no successful attacks, with $P(M) = 0$.}
\label{tbl:avgqueries-RF}
\vfill
%\end{table}

%\end{figure}
%\end{minipage}
\end{figure}
%}


==> images/nn_mattbl.tex <==
% !TEX root = ../ms.tex
\begin{figure}[t]
%\begin{minipage}[\textheight]{\linewidth}
%\begin{figure}[t] 
	\centering

\textsc{Neural Network}

\subfloat[][Random Pixel Image Perturb. Attack Coverage]{\includegraphics[width=0.978\columnwidth]{images/rand_image_mats_nn.pdf}}

\subfloat[][VAE Latent Space Perturb. Attack Coverage]{\includegraphics[width=0.978\columnwidth]{images/vae_tabular_mats_nn.pdf}}

    % \textsc{Neural Network}\par\medskip
    % \begin{subfigure}[t]{0.42\textwidth}
    %     \centering
    %     \text{Random Pixel Image Perturb.}
    %     \text{Attack Coverage}\par\medskip
    %     \includegraphics[width=\textwidth]{images/rand_image_mats_nn.eps}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.42\textwidth}
    %     \centering
    %     \text{VAE Latent Space Perturb.}
    %     \text{Attack Coverage}\par\medskip 
    %     \includegraphics[width=\textwidth]{images/vae_tabular_mats_nn.eps}
    % \end{subfigure}

%    \captionsetup{width=\textwidth}
    \captionof{figure}{Coverage maps for the Facenet-NN classifier. Cells denote authentication success for each adversary--victim pair. Lighter cells denote unsuccessful queries shaded by the model's confidence, when available. }

    % \caption{Coverage heatmaps for each experiment across both face image perturbation techniques, with an adversary's knowledge set to a random 30\% subset of all registered names. Cells denote authentication success for each adversary--victim pair.}
    % Without LIME, the VAE appraoch is more successful than random perturbations. In both cases, the LIME-assisted attack yields higher attack coverage. 
	\label{fig:nn_mats}
\par\medskip
\hfill

%\begin{table}[b]
% \setlength\tabcolsep{3pt}
%\footnotesize
\centering
%\begin{subtable}{0.5\textwidth}
%\centering

\begin{footnotesize}
\begin{tabular}{|c||c|c|c|}
%\begin{tabular}{|c||cc|cc|cc|}
%\hline
% & \multicolumn{3}{c|}{Defenses} \\\hline
%
\multicolumn{4}{c}{Random Pixel Image Perturb. Attack} \\\hline
          & No Defense                & Random Defense                & All Defense\\\hline\hline
%           & Defense & Defense & Defenses \\\hline\hline
 Random   &  13.21 $\pm$ 7.16  &   ---                         &   ---   \\
           & $P(M)=93$\% & & \\\hline
 Ablation &  140 $\pm$ 45.56    &   136.4 $\pm$ 53.47    &   164.75 $\pm$ 67.33   \\
  & $P(M)=60$\% & $P(M)=67$\% & $P(M)=27$\% \\\hline
 LIME     &  130.23 $\pm$ 44.38 &   160.73 $\pm$  63.02  &   142.89 $\pm$ 63.58   \\
  & $P(M)=87$\% & $P(M)=73$\% & $P(M)=60$\% \\\hline
\multicolumn{4}{c}{} \\
\multicolumn{4}{c}{VAE Latent Space Perturb. Attack} \\\hline
          & No Defense                & Random Defense               & All Defense\\\hline\hline
%           & Defense & Defense & Defenses \\\hline\hline
 Random   &  11.21 $\pm$ 0.41   &   ---                        &   ---   \\
  & $P(M)=93$\% & & \\\hline
 Ablation &  104.08 $\pm$ 25.69 &   127 $\pm$ 50.71     &   155.88 $\pm$ 46.10  \\
  & $P(M)=87$\% & $P(M)=87$\% & $P(M)=53$\% \\\hline
 LIME     &  108.23 $\pm$ 23.18 &   118.69 $\pm$ 29.27  &   144.43 $\pm$ 58.78  \\
  & $P(M)=87$\% & $P(M)=87$\% & $P(M)=93$\% \\\hline
%
\end{tabular}
\end{footnotesize}
\par\medskip

\captionof{table}{The average number of adversarial queries before success in each of three experiments, 
against the Facenet-NN classifier and with varying level of defenses at 30\% knowledge.
Dashes indicate no successful attacks, with $P(M) = 0$.}
\label{tbl:avgqueries-NN}
\vfill

%\end{minipage}
\end{figure}


==> images/svm_mattbl.tex <==
% !TEX root = ../ms.tex

\begin{figure}[t]
%\begin{minipage}{\linewidth}
%\parbox[t]{0.48\textwidth}{
%\begin{figure}[t]
%\begin{figure}[t] 
\centering

\textsc{Support Vector Machine}

\subfloat[][Random Pixel Image Perturb. Attack Coverage]{\includegraphics[width=0.978\columnwidth]{images/rand_image_mats_svm.pdf}}

\subfloat[][VAE Latent Space Perturb. Attack Coverage]{\includegraphics[width=0.978\columnwidth]{images/vae_tabular_mats_svm.pdf}}

    % \begin{subfigure}[t]{0.42\textwidth}
    %     \centering
    % 	\text{Random Pixel Image Perturb.}
    %     \text{Attack Coverage}\par\medskip
    % 	\includegraphics[width=\textwidth]{images/rand_image_mats_svm.eps}
    % 	% \textbf{(a)}\par\medskip
    % \end{subfigure}
    % \begin{subfigure}[t]{0.42\textwidth}
    %     \centering
    % 	\text{VAE Latent Space Perturb.}
    %     \text{Attack Coverage}\par\medskip
    % 	\includegraphics[width=\textwidth]{images/vae_tabular_mats_svm.eps}
    % 	% \textbf{(b)}\par\medskip
    % \end{subfigure}

%\captionsetup{width=\textwidth}
\captionof{figure}{Coverage maps for the Facenet-SVM classifier. Cells denote authentication success for each adversary--victim pair. Lighter cells denote unsuccessful queries shaded by the model's confidence, when available. }
\label{fig:svm_mats}
	% Without LIME, the VAE appraoch is more successful than random perturbations. In both cases, the LIME-assisted attack yields higher attack coverage. 
%\end{figure}
%\par\medskip
\hfill

%\begin{table}[b]

% \setlength\tabcolsep{3pt}

%\footnotesize
\centering
%\begin{subtable}{0.5\textwidth}
%\centering
\par\medskip

\begin{footnotesize}
\begin{tabular}{|c||c|c|c|}
%\begin{tabular}{|c||cc|cc|cc|}
%\hline
% & \multicolumn{3}{c|}{Defenses} \\\hline
\multicolumn{4}{c}{Random Pixel Image Perturb. Attack} \\\hline
 & No Defense & Random Defense & All Defense\\\hline\hline
% & Defense & Defense & Defenses \\\hline\hline
 % & No Defense  & Random Defense & All Defenses \\\hline\hline
 Random & 22 $\pm$ 13.68 & ---  & --- \\
 &  $P(M)=87$\% & & \\\hline
 Ablation & 129.5 $\pm$ 38.56 & 131 $\pm$ 0 & --- \\
 & $P(M)=40$\% & $P(M)=7$\% & \\\hline
 LIME & 114.67 $\pm$ 25.99 & 124.75 $\pm$ 25.91 & 152 $\pm$ 0 \\
 & $P(M)=80$\% & $P(M)=27$\% & $P(M)=7$\% \\\hline
\multicolumn{4}{c}{} \\
\multicolumn{4}{c}{VAE Latent Space Perturb. Attack} \\\hline
 & No Defense & Random Defense & All Defense\\\hline\hline
% & Defense & Defense & Defenses \\\hline\hline

 Random & 31.21 $\pm$ 16.42 & ---  & --- \\
  & $P(M)=93$\% & & \\\hline
 Ablation & 102.62 $\pm$ 23.56 & 90.46 $\pm$ 12.35 & 113.6 $\pm$ 13.88 \\
  & $P(M)=87$\% & $P(M)=87$\% & $P(M)=33$\% \\\hline
 LIME & 100.54 $\pm$ 25.66 & 104.69 $\pm$ 22.03 & 124 $\pm$ 19.03 \\
  & $P(M)=87$\% & $P(M)=87$\% & $P(M)=20$\% \\\hline
% & \multicolumn{2}{c|}{No Defense}  & \multicolumn{2}{c|}{Random Defense} & \multicolumn{2}{c|}{All Defenses} \\\hline\hline
% Random & 22 $\pm$ 13.68 & 87\% & --- & & --- & \\\hline
% Ablation & 129.5 $\pm$ 38.56 & 40\% & 131 $\pm$ 0 & 7\% & --- & \\\hline
% LIME & 114.67 $\pm$ 25.99 & 20\% & 124.75 $\pm$ 25.91 & 27\% & 152 $\pm$ 0 & 7\% \\\hline
\end{tabular}
\end{footnotesize}
\par\medskip

%\caption{Random Pixel Image Perturb. Attack}
%\caption{SVM: Random Pixel Image Perturb. Attack}
%\label{tbl:queries-randomSVM}
%\end{subtable}
%\end{table}
%\\
%\begin{table}[t]
%\begin{subtable}{0.5\textwidth}
%\centering
%\text{VAE Latent Space Perturb. Attack}\par\medskip
%\begin{footnotesize}
%\begin{tabular}{|c||c|c|c|c}
%\begin{tabular}{|c||cc|cc|cc|}
%\hline
% & \multicolumn{3}{c|}{Defenses} \\\hline
% & No Defense  & Random Defense & All Defenses \\\hline\hline
% Random & 31.21 $\pm$ 16.42 (93\%) & ---  & --- \\\hline
% Ablation & 102.62 $\pm$ 23.56 (87\%) & 90.46 $\pm$ 12.35 (87\%) & 113.6 $\pm$ 13.88 (33\%) \\\hline
% LIME & 100.54 $\pm$ 25.66 (87\%) & 104.69 $\pm$ 22.03 (87\%) & 124 $\pm$ 19.03 (20\%) \\\hline
% & \multicolumn{2}{c|}{No Defense}  & \multicolumn{2}{c|}{Random Defense} & \multicolumn{2}{c|}{All Defenses} \\\hline\hline
% Random & 31.21 $\pm$ 16.42 & 93\% & --- & & --- & \\\hline
% Ablation & 102.62 $\pm$ 23.56 & 87\% & 90.46 $\pm$ 12.35 & 87\% & 113.6 $\pm$ 13.88 & 33\% \\\hline
% LIME & 100.54 $\pm$ 25.66 & 87\% & 104.69 $\pm$ 22.03 & 87\% & 124 $\pm$ 19.03 & 20\% \\\hline
%\end{tabular}
%\end{footnotesize}
%\caption{VAE Latent Space Perturb. Attack}
%\caption{SVM: VAE Latent Space Perturb. Attack}
%\label{tbl:queries-vaeSVM}
%\end{subtable}
\captionof{table}{The average number of adversarial queries before success in each of threee experiments,
against the Facenet-SVM classifier and with varying level of defenses at 30\% knowledge.
Dashes indicate no successful attacks, with $P(M) = 0$.}
\label{tbl:avgqueries-SVM}
%\vfill
%\end{table}

%\end{figure}
%\end{minipage}
\end{figure}
%}


==> tables/face_tab_svm.tex <==
% !TEX root = ../ms.tex
\begin{table}[t]
\setlength\tabcolsep{3pt}
\footnotesize
\centering
\begin{subtable}{0.5\textwidth}
\centering
\begin{tabular}{|c||c|c|c|}
%\begin{tabular}{|c||cc|cc|cc|}
\hline
% & \multicolumn{3}{c|}{Defenses} \\\hline
 & No Defense  & Random Defense & All Defenses \\\hline\hline
 Random & 22 $\pm$ 13.68 (87\%) & ---  & --- \\\hline
 Ablation & 129.5 $\pm$ 38.56 (40\%) & 131 $\pm$ 0 (7\%) & --- \\\hline
 LIME & 114.67 $\pm$ 25.99 (80\%) & 124.75 $\pm$ 25.91 (27\%) & 152 $\pm$ 0 (7\%) \\\hline
% & \multicolumn{2}{c|}{No Defense}  & \multicolumn{2}{c|}{Random Defense} & \multicolumn{2}{c|}{All Defenses} \\\hline\hline
% Random & 22 $\pm$ 13.68 & 87\% & --- & & --- & \\\hline
% Ablation & 129.5 $\pm$ 38.56 & 40\% & 131 $\pm$ 0 & 7\% & --- & \\\hline
% LIME & 114.67 $\pm$ 25.99 & 20\% & 124.75 $\pm$ 25.91 & 27\% & 152 $\pm$ 0 & 7\% \\\hline
\end{tabular}
%\caption{Random Pixel Image Perturb. Attack}
\caption{SVM: Random Pixel Image Perturb. Attack}
\label{tbl:queries-randomSVM}
\end{subtable}
%\end{table}
\\
%\begin{table}[t]
\begin{subtable}{0.5\textwidth}
\centering
\begin{tabular}{|c||c|c|c|c}
%\begin{tabular}{|c||cc|cc|cc|}
\hline
% & \multicolumn{3}{c|}{Defenses} \\\hline
 & No Defense  & Random Defense & All Defenses \\\hline\hline
 Random & 31.21 $\pm$ 16.42 (93\%) & ---  & --- \\\hline
 Ablation & 102.62 $\pm$ 23.56 (87\%) & 90.46 $\pm$ 12.35 (87\%) & 113.6 $\pm$ 13.88 (33\%) \\\hline
 LIME & 100.54 $\pm$ 25.66 (87\%) & 104.69 $\pm$ 22.03 (87\%) & 124 $\pm$ 19.03 (20\%) \\\hline
% & \multicolumn{2}{c|}{No Defense}  & \multicolumn{2}{c|}{Random Defense} & \multicolumn{2}{c|}{All Defenses} \\\hline\hline
% Random & 31.21 $\pm$ 16.42 & 93\% & --- & & --- & \\\hline
% Ablation & 102.62 $\pm$ 23.56 & 87\% & 90.46 $\pm$ 12.35 & 87\% & 113.6 $\pm$ 13.88 & 33\% \\\hline
% LIME & 100.54 $\pm$ 25.66 & 87\% & 104.69 $\pm$ 22.03 & 87\% & 124 $\pm$ 19.03 & 20\% \\\hline
\end{tabular}
%\caption{VAE Latent Space Perturb. Attack}
\caption{SVM: VAE Latent Space Perturb. Attack}
\label{tbl:queries-vaeSVM}
\end{subtable}
%\label{tbl:avgqueries}
%\caption{SVM: The average number of adversarial queries before success in each of three experiments
%and varying level of defenses at 30\% knowledge.
%In parentheses is calculated probability $P(M)$ based on attack coverage for the experiment.
%Dashes indicate no successful attacks, with $P(M) = 0$.}
%\end{table}
%
%%%%%%%%%%
%
%\begin{table}[t]
\begin{subtable}{0.5\textwidth}
\centering
\begin{tabular}{|c||c|c|c|}
\hline
          & No Defense                 & Random Defense                & All Defenses \\\hline\hline
 Random   &  13.21 $\pm$ 7.16 (93\%)   &   ---                         &   ---   \\\hline
 Ablation &  140 $\pm$ 45.56 (60\%)    &   136.4 $\pm$ 53.47 (67\%)    &   164.75 $\pm$ 67.33 (27\%)   \\\hline
 LIME     &  130.23 $\pm$ 44.38 (87\%) &   160.73 $\pm$  63.02 (73\%)  &   142.89 $\pm$ 63.58 (60\%)   \\\hline
\end{tabular}
%\caption{Random Pixel Image Perturb. Attack}
\caption{Neural Network: Random Pixel Image Perturb. Attack}
\label{tbl:queries-randomNN}
\end{subtable}
\\
\begin{subtable}{0.5\textwidth}
\centering
\begin{tabular}{|c||c|c|c|c}
\hline
          & No Defense                 & Random Defense               & All Defenses \\\hline\hline
 Random   &  11.21 $\pm$ 0.41 (93\%)   &   ---                        &   ---   \\\hline
 Ablation &  104.08 $\pm$ 25.69 (87\%) &   127 $\pm$ 50.71 (87\%)     &   155.88 $\pm$ 46.10 (53\%)  \\\hline
 LIME     &  108.23 $\pm$ 23.18 (87\%) &   118.69 $\pm$ 29.27 (87\%)  &   144.43 $\pm$ 58.78 (93\%)  \\\hline
\end{tabular}
%\caption{VAE Latent Space Perturb. Attack}
\caption{Neural Network: VAE Latent Space Perturb. Attack}
\label{tbl:queries-vaeNN}
\end{subtable}
%\label{tbl:avgqueriesNN}
%\caption{Neural Net: The average number of adversarial queries before success in each of three experiments
%and varying level of defenses at 30\% knowledge.
%In parentheses is calculated probability $P(M)$ based on attack coverage for the experiment.
%Dashes indicate no successful attacks, with $P(M) = 0$.}
%\end{table}

%%%%%%%%%%
%
%\begin{table}[t]
\begin{subtable}{0.5\textwidth}
\centering
\begin{tabular}{|c||c|c|c|}
\hline
          & No Defense                  & Random Defense               & All Defenses \\\hline\hline
 Random   &  94 $\pm$ 64.82 (73\%)      &  ---                         &  ---  \\\hline
 Ablation &  152.47 $\pm$ 84.10 (100\%) &  162.33 $\pm$ 67.12 (100\%)  &  107.5 $\pm$ 18.27 (93\%)   \\\hline
 LIME     &  120.67 $\pm$ 80.49 (100\%) &  118.53 $\pm$ 26.26 (100\%)  &  123.71 $\pm$ 24.58 (93\%)   \\\hline
\end{tabular}
%\caption{Random Pixel Image Perturb. Attack}
\caption{Random Forest: Random Pixel Image Perturb. Attack}
\label{tbl:queries-randomRF}
\end{subtable}
\\
\begin{subtable}{0.5\textwidth}
\centering
\begin{tabular}{|c||c|c|c|c}
\hline
          & No Defense                 & Random Defense               & All Defenses \\\hline\hline
 Random   &  84.11 $\pm$ 66.32 (60\%)  &  ---                         &  ---    \\\hline
 Ablation &  125.23 $\pm$ 38.94 (87\%) &  112.58 $\pm$ 50.37 (80\%)   &  102.43 $\pm$ 23.63 (93\%)   \\\hline
 LIME     &  132.43 $\pm$ 35.04 (93\%) &  99 $\pm$ 21.51 (80\%)       &  112.29 $\pm$ 39.27 (93\%)   \\\hline
\end{tabular}
%\caption{VAE Latent Space Perturb. Attack}
\caption{Random Forest: VAE Latent Space Perturb. Attack}
\label{tbl:queries-vaeRF}
\end{subtable}
%\label{tbl:avgqueriesRF}
\caption{The average number of adversarial queries before success in each of three experiments,
against three different models and with varying level of defenses at 30\% knowledge.
In parentheses is calculated probability $P(M)$ based on attack coverage for the experiment.
Dashes indicate no successful attacks, with $P(M) = 0$.}
\label{tbl:avgqueries}
\end{table}



==> tables/facepp_que_tab.tex <==
% !TEX root = ../ms.tex
\begin{table}[t]
\setlength\tabcolsep{3pt}
\footnotesize
\centering
\begin{tabular}{|c||c|}
\hline
 Random   & ---  \\\hline
 QuickStart & 163.88 $\pm$ 48.35 (53\%)  \\\hline
 QuickStart+LIME & 155.11 $\pm$ 39.63 (60\%)  \\\hline
\end{tabular}
\caption{The average number of adversarial queries before success in each of three experiments,
testing against Face++ API at 30\% knowledge.
In parentheses is calculated probability $P(M)$ based on attack coverage for the experiment.
Dashes indicate no successful attacks, with $P(M) = 0$.}
\label{tbl:ppqueries}
\end{table}


